Zooming in on the Universe: In Search of Quantum Spacetime

This thesis investigates low-dimensional models of nonperturbative quantum gravity, with a special focus on Causal Dynamical Triangulations (CDT). We define the so-called curvature profile, a new quantum gravitational observable based on the quantum Ricci curvature. We subsequently study its coarse-graining capabilities on a class of regular, two-dimensional polygons with isolated curvature singularities, and we determine the curvature profile of (1+1)-dimensional CDT with toroidal topology. Next, we focus on CDT in 2+1 dimensions, intvestigating the behavior of the two-dimensional spatial slice geometries. We then turn our attention to matrix models, exploring a differential reformulation of the integrals over one- and two-matrix ensembles. Finally, we provide a hands-on introduction to computer simulations of CDT quantum gravity.

==> chapters/cdt.tex <==
\chapter{CDT quantum gravity}\label{ch:cdt}


==> chapters/matrix-models.tex <==
%!TEX root = ../thesis.tex
\chapter{Introduction to matrix models}\label{ch:matrix-models}



==> figures/defects/dbocta <==
dbocta = {{-1.47, 0., 1.5653424687362376}, {-1.4688666832738626, 
      -0.05386446722144213, 1.5654548190121158}, {-1.465468480587698, 
      -0.10764587933860326, 1.5657909063694648}, {-1.4598106317237416, 
      -0.16126130931215324, 1.5663478828410642}, {-1.4519018606748526, 
      -0.21462808603519673, 1.5671210011451473}, {-1.4417543621927487, 
      -0.2676639218061279, 1.5681033748371194}, {-1.4293837829845844, 
      -0.32028703921030216, 1.5692867426694581}, {-1.4148091975868615, 
      -0.3724162972148819, 1.5706602607959617}, {-1.3980530789538756, 
      -0.4239713162824279, 1.5722110750045055}, {-1.3791412638060516, 
      -0.4748726023103203, 1.5739225157971375}, {-1.3581029127915913, 
      -0.5250416692049031, 1.574140662521187}, {-1.3349704655228694, 
      -0.5744011599013513, 1.5741386466348473}, {-1.3097795905569007, 
      -0.6228749656426582, 1.5741311391038093}, {-1.2825691303970117, 
      -0.6703883433338221, 1.5741191894903375}, {-1.2533810416005158, 
      -0.7168680307902816, 1.5741033156476598}, {-1.2222603300847414, 
      -0.7622423597028942, 1.5740839993807116}, {-1.1892549817311728, 
      -0.8064413661452732, 1.5740616698138634}, {-1.1544158883946951, 
      -0.8493968984530921, 1.5740362934568657}, {-1.1177967694320454, 
      -0.8910427223090118, 1.5740083194228072}, {-1.0794540888704578, 
      -0.931314622871196, 1.5739780200435942}, {-1.0394469683442247, 
      -0.970150503787943, 1.5739455077214206}, {-0.9978370959334244, 
      -1.0074904829457605, 1.573911140659381}, {-0.9546886310453699, 
      -1.0432769848032424, 1.573875175967482}, {-0.9100681054854559, 
      -1.077454829168382, 1.573837917307207}, {-0.8640443208699355, 
      -1.1099713162824276, 1.5737997482296335}, {-0.8166882425388152, 
      -1.140776308079092, 1.5737610765216334}, {-0.7680728901324447, 
      -1.1698223054938146, 1.5737221402707064}, {-0.7182732250005237, 
      -1.1970645217038778, 1.5736834036048102}, {-0.6673660346171338, 
      -1.2224609511864406, 1.5736453507150725}, {-0.6154298141800193, 
      -1.2459724344880112, 1.5736082519850112}, {-0.5625446455766819, 
      -1.2675627186054852, 1.573572469344024}, {-0.5087920739039147, 
      -1.2871985128856482, 1.5735386564767344}, {-0.45425498173117274, 
      -1.3048495403569504, 1.5735071335798285}, {-0.39901746130165916, 
      -1.320488584414404, 1.5734782601413349}, {-0.3431646848681809, 
      -1.3340915307856123, 1.5734524237551333}, {-0.28678277336370855, 
      -1.345637404713232, 1.5734299718687452}, {-0.22995866360913939, 
      -1.3551084032965288, 1.5734112545718897}, {-0.17277997426302133, 
      -1.3624899229421588, 1.573396416863597}, {-0.11533487071993208, 
      -1.3677705818818515, 1.5733855936232013}, {-0.05771192916583085, 
      -1.3709422377222718, 1.5733790851299607}, {0., -1.3719999999999999, 
      1.573376890152805}, {-1.4849999999999999, 0., 1.5699777531996064}, 
     {-1.4838551188174733, -0.05441410464206909, 1.5700884978027319}, 
     {-1.4804222405936949, -0.10874430667879308, 1.5704198164434993}, 
     {-1.4747066585780655, -0.16290683287656296, 1.5709687459602877}, 
     {-1.4667171857837795, -0.21681816854575997, 1.571730498228485}, 
     {-1.4564661413987972, -0.2703951863143537, 1.5726977775539683}, 
     {-1.4439693317905495, -0.3235552743042849, 1.5738612872230981}, 
     {-1.4292460261336664, -0.3762164635129929, 1.5744715879324154}, 
     {-1.412318926698303, -0.42829755420367716, 1.574469068673905}, 
     {-1.393214133844889, -0.4797182411094052, 1.574464536330316}, 
     {-1.3719611057792607, -0.5303992372580144, 1.5744578154065407}, 
     {-1.3485926131302457, -0.5802623962268753, 1.5744490980672956}, 
     {-1.3231446884197264, -0.6292308326390118, 1.5744384371309117}, 
     {-1.2956565705031038, -0.6772290407147795, 1.5744258692915925}, 
     {-1.2661706440658271, -0.724183010696305, 1.5744113235988693}, 
     {-1.2347323742692795, -0.7700203429651686, 1.5743949285525425}, 
     {-1.201390236646797, -0.8146703596773678, 1.5743765125690323}, 
     {-1.1661956423579063, -0.8580642137434298, 1.5743562216755351}, 
     {-1.1292028589160459, -0.9001349949856344, 1.5743340337849472}, 
     {-1.0904689265119931, -0.9408178333086573, 1.5743100142004256}, 
     {-1.050053570062023, -0.9800499987245547, 1.574284307249994}, 
     {-1.0080191071164184, -1.01777099807786, 1.574257066198042}, 
     {-0.9644303517703228, -1.053922668321643, 1.5742284461207299}, 
     {-0.9193545147251034, -1.0884492662007124, 1.5741986545877396}, 
     {-0.8728610996543226, -1.121297554203677, 1.5741679465049225}, 
     {-0.8250217960341092, -1.1524168826513277, 1.5741365879118563}, 
     {-0.775910368603184, -1.181759267794772, 1.574104862022999}, 
     {-0.725602543622978, -1.209279465802897, 1.5740731376309063}, 
     {-0.674175892113227, -1.2349350425250778, 1.574041779335595}, 
     {-0.6217097102430807, -1.2586864389215624, 1.5740109936581024}, 
     {-0.5682848970621583, -1.2804970320606432, 1.5739812761765963}, 
     {-0.5139838297600771, -1.300333191588563, 1.5739529345698617}, 
     {-0.45889023664679696, -1.3181643315850826, 1.57392646736494}, 
     {-0.4030890680496353, -1.3339629577247551, 1.573902144484692}, 
     {-0.34666636532601947, -1.3477047096711796, 1.5738803211938048}, 
     {-0.28970912819395045, -1.3593683986388774, 1.5738612425359764}, 
     {-0.23230518058474287, -1.368936040064861, 1.5738454134888464}, 
     {-0.1745430352248889, -1.3763928813395279, 1.573832793289643}, 
     {-0.11651175715584974, -1.3817274245541153, 1.5738235638774933}, 
     {-0.058300826402216885, -1.3849314442296419, 1.573818078178106}, 
     {0., -1.386, 1.57381617538344}, {-1.5, 0., 0.15916459079271955*
       Re[(0. + NIntegrate[j11$15187102*j21$15187102*
            dd[c1$15187102[[1]][t][[1]], c1$15187102[[1]][t][[2]], 
             c2$15187102[[1]][u][[1]], c2$15187102[[1]][u][[2]], (2*Pi)/3], 
           b11$15187102, b21$15187102, AccuracyGoal -> acc$15187102] + 
          NIntegrate[j11$15187102*j22$15187102*dd[c1$15187102[[1]][t][[1]], 
             c1$15187102[[1]][t][[2]], c2$15187102[[2]][u][[1]], 
             c2$15187102[[2]][u][[2]], (2*Pi)/3], b11$15187102, b22$15187102, 
           AccuracyGoal -> acc$15187102])/(0. + NIntegrate[m1$15187335, 
           {t, 0 + 1/400000000, 1 - 1/400000000}, AccuracyGoal -> 
            acc$15187335])]}, {-1.4988435543610843, -0.05496374206269605, 
      1.574608256693452}, {-1.495376000599692, -0.10984273401898291, 
      1.5746054733293462}, {-1.4896026854323894, -0.16455235644097269, 
      1.5746033227882323}, {-1.4815325108927067, -0.2190082510563232, 
      1.5746015475888246}, {-1.4711779206048456, -0.2731264508225795, 
      1.5745999050826036}, {-1.4585548805965147, -0.32682350939826754, 
      1.5745983659926968}, {-1.443682854680471, -0.38001662981110396, 
      1.5745966055002323}, {-1.4265847744427302, -0.4326237921249264, 
      1.5745947235959008}, {-1.4072870038837262, -0.4845638799084901, 
      1.5745926283852547}, {-1.38581929876693, -0.5357568053111257, 
      1.5745898689287807}, {-1.3622147607376218, -0.5861236325523993, 
      1.5745863053032012}, {-1.336509786282552, -0.6355866996353655, 
      1.5745817408899683}, {-1.3087440106091957, -0.6840697380957369, 
      1.5745766407380155}, {-1.2789602465311385, -0.7314979906023282, 
      1.5745699883224695}, {-1.2472044184538178, -0.777798326227443, 
      1.5745619163652387}, {-1.2135254915624212, -0.8228993532094624, 
      1.5745526021196732}, {-1.1779753963211175, -0.8667315290337675, 
      1.574541788680504}, {-1.1406089484000463, -0.909227267662257, 
      1.5745294839241761}, {-1.1014837641535284, -0.9503210437461185, 
      1.5745153484908334}, {-1.0606601717798212, -0.9899494936611664, 
      1.574499692129382}, {-1.0182011182994126, -1.0280515132099597, 
      1.5744825283186876}, {-0.9741720724952755, -1.0645683518400433, 
      1.5744639233819706}, {-0.928640923964751, -1.0994437032330429, 
      1.574444027199789}, {-0.8816778784387097, -1.1326237921249263, 
      1.5744230090519704}, {-0.8333553495294033, -1.1640574572235634, 
      1.5744010398279733}, {-0.7837478470739232, -1.1936962300957292, 
      1.5743784831479508}, {-0.7329318622454324, -1.221494409901916, 
      1.574355511511606}, {-0.6809857496093202, -1.247409133863715, 
      1.574332356154084}, {-0.6279896063061422, -1.2714004433551136, 
      1.5743094325190434}, {-0.5740251485476346, -1.2934313455158013, 
      1.5742868388195328}, {-0.5191755856162394, -1.3134678702914777, 
      1.5742652574902547}, {-0.4635254915624212, -1.3314791228132148, 
      1.574244833316879}, {-0.4071606747976114, -1.3474373310351062, 
      1.574225968097559}, {-0.3501680457838581, -1.3613178885567472, 
      1.5742089047293102}, {-0.2926354830241924, -1.3730993925645225, 
      1.5741939663025855}, {-0.23465169756034632, -1.3827636768331928, 
      1.574181488299349}, {-0.17630609618675647, -1.3902958397368967, 
      1.5741714840061938}, {-0.11768864359176742, -1.3956842672263792, 
      1.5741641710422363}, {-0.05888972363860291, -1.398920650737012, 
      1.5741597606707332}, {0., -1.4, 1.5741582632102993}, 
     {-1.5150000000000001, 0., 1.574598225275804}, {-1.5138319899046953, 
      -0.055513379483323015, 1.5745981623285172}, {-1.510329760605689, 
      -0.11094116135917274, 1.57459792070071}, {-1.5044987122867133, 
      -0.1661978800053824, 1.574597609978793}, {-1.4963478360016338, 
      -0.22119833356688645, 1.574597218676593}, {-1.4858896998108941, 
      -0.27585771533080533, 1.5745968271688024}, {-1.47314042940248, 
      -0.3300917444922502, 1.5745964339026386}, {-1.4581196832272756, 
      -0.383816796109215, 1.5745961195153766}, {-1.4408506221871575, 
      -0.43695003004617566, 1.5745958745193163}, {-1.4213598739225635, 
      -0.489409518707575, 1.5745957458002862}, {-1.3996774917545993, 
      -0.541114373364237, 1.5745956121250746}, {-1.375836908344998, 
      -0.5919848688779233, 1.57459561015956}, {-1.3498748841453774, 
      -0.6419425666317192, 1.574595855254222}, {-1.3218314507152875, 
      -0.6909104354766943, 1.5745960535119876}, {-1.2917498489964498, 
      -0.7388129705083515, 1.5745963457430328}, {-1.259676462638356, 
      -0.7855763094897175, 1.574596720215511}, {-1.2256607464780453, 
      -0.831128346741557, 1.5745972899329832}, {-1.1897551502843287, 
      -0.8753988443241052, 1.574597898164988}, {-1.1520150378840468, 
      -0.9183195403388796, 1.5745981570204985}, {-1.1124986017950638, 
      -0.9598242541835796, 1.574597189999572}, {-1.0712667734976193, 
      -0.999848988597778, 1.5745945774351162}, {-1.0283831294824068, 
      -1.0383320283420594, 1.574589964430024}, {-0.9839137932202282, 
      -1.0752140353584436, 1.5745836370797242}, {-0.9379273332043985, 
      -1.1104381402653734, 1.5745760439899823}, {-0.8904946572230968, 
      -1.1439500300461756, 1.5745666633954642}, {-0.8416889030246973, 
      -1.175698031795799, 1.5745561656672762}, {-0.7915853255446624, 
      -1.2056331923966865, 1.5745445560250548}, {-0.7402611808678867, 
      -1.2337093540009352, 1.574531878041238}, {-0.6877956071054134, 
      -1.2598832252023522, 1.5745186240038396}, {-0.6342695023692037, 
      -1.2841144477886648, 1.5745048884960535}, {-0.579765400033111, 
      -1.3063656589709594, 1.5744905912756102}, {-0.5243673414724018, 
      -1.3266025489943924, 1.5744767630486753}, {-0.4681607464780454, 
      -1.344793914041347, 1.5744633928017882}, {-0.41123228154558755, 
      -1.3609117043454573, 1.5744507279709372}, {-0.3536697262416967, 
      -1.3749310674423147, 1.5744392334589534}, {-0.29556183785443435, 
      -1.3868303864901677, 1.5744289557637927}, {-0.23699821453594977, 
      -1.3965913136015247, 1.5744203556291054}, {-0.17806915714862404, 
      -1.4041987981342656, 1.5744134634435305}, {-0.1188655300276851, 
      -1.409641109898643, 1.5744082762603124}, {-0.05947862087498894, 
      -1.4129098572443821, 1.5744051787742739}, 
     {0., -1.414, 1.574404033459401}}
 
Attributes[m1$15187335] = {Temporary}
 
m1$15187335 = Sqrt[1.7777777777777777*
       Cos[0.6666666666666666*(0. - (\[Tau] /. {}[[1]]) + 
           t*(0. + 2*(\[Tau] /. {}[[1]])))]^2*(0. + 2*(\[Tau] /. {}[[1]]))^
        2 + 1.7777777777777777*(0. + 2*(\[Tau] /. {}[[1]]))^2*
       Sin[0.6666666666666666*(0. - (\[Tau] /. {}[[1]]) + 
           t*(0. + 2*(\[Tau] /. {}[[1]])))]^2]
 
Attributes[acc$15187335] = {Temporary}
 
acc$15187335 = 10
 
Attributes[j11$15187102] = {Temporary}
 
j11$15187102 = Sqrt[1.7777777777777777*
       Cos[0.6666666666666666*(0. - (\[Tau] /. {}[[1]]) + 
           t*(0. + 2*(\[Tau] /. {}[[1]])))]^2*(0. + 2*(\[Tau] /. {}[[1]]))^
        2 + 1.7777777777777777*(0. + 2*(\[Tau] /. {}[[1]]))^2*
       Sin[0.6666666666666666*(0. - (\[Tau] /. {}[[1]]) + 
           t*(0. + 2*(\[Tau] /. {}[[1]])))]^2]
 
Attributes[j21$15187102] = {Temporary}
 
j21$15187102 = Sqrt[0.27415567780803773*
       (4.*Cos[0.6666666666666666*(-0.7853981633974483 + 1.5707963267948966*
              u)] + Sqrt[-12. + 16.*Cos[0.6666666666666666*(
                -0.7853981633974483 + 1.5707963267948966*u)]^2])^2 + 
      0.25*(-4.1887902047863905*Sin[0.6666666666666666*(-0.7853981633974483 + 
             1.5707963267948966*u)] - (16.755160819145562*
           Cos[0.6666666666666666*(-0.7853981633974483 + 1.5707963267948966*
               u)]*Sin[0.6666666666666666*(-0.7853981633974483 + 
              1.5707963267948966*u)])/Sqrt[-12. + 
            16.*Cos[0.6666666666666666*(-0.7853981633974483 + 
                 1.5707963267948966*u)]^2])^2]
 
dd[r1_, \[Theta]1_, r2_, \[Theta]2_, \[Alpha]_] := 
    If[Inequality[0, LessEqual, Abs[\[Theta]2 - \[Theta]1], Less, Pi], 
     Sqrt[r1^2 + r2^2 - 2*r1*r2*Cos[(1 - \[Alpha]/(2*Pi))*
          (\[Theta]2 - \[Theta]1)]], 
     Sqrt[r1^2 + r2^2 - 2*r1*r2*Cos[(1 - \[Alpha]/(2*Pi))*
          (2*Pi - Abs[\[Theta]2 - \[Theta]1])]]]
 
dd[p1_, p2_, \[Alpha]_] := dd[p1[[1]], p1[[2]], p2[[1]], p2[[2]], \[Alpha]]
 
\[Alpha] = (2*Pi)/3
 
p1 = {-0.5, 1.414}
 
p2 = {0.5, 1.414}
 
Attributes[c1$15187102] = {Temporary}
 
c1$15187102 = {{rp$15187103[t1$15187103[#1]], t1$15187103[#1]} & , 
     {rm$15187103[t2$15187103[#1]], t2$15187103[#1]} & }
 
Attributes[rp$15187103] = {Temporary}
 
rp$15187103[t$_] := \[Rho] /. s$15187103[[2]] /. \[Tau] -> t$
 
Attributes[t$] = {Temporary}
 
Attributes[s$15187103] = {Temporary}
 
s$15187103 = {{\[Rho] -> 0.}, 
     {\[Rho] -> 2.*Cos[0.6666666666666666*(0. + \[Tau])]}}
 
Attributes[t1$15187103] = {Temporary}
 
t1$15187103[t$_] := tr$15187103 + (tl$15187103 - tr$15187103)*t$
 
Attributes[tr$15187103] = {Temporary}
 
tr$15187103 = 0. - (\[Tau] /. {}[[1]])
 
Attributes[tl$15187103] = {Temporary}
 
tl$15187103 = \[Tau] /. {}[[1]]
 
Attributes[rm$15187103] = {Temporary}
 
rm$15187103[t$_] := \[Rho] /. s$15187103[[1]] /. \[Tau] -> t$
 
Attributes[t2$15187103] = {Temporary}
 
t2$15187103[t$_] := tl$15187103 + (tr$15187103 - tl$15187103)*(t$ - 1)
 
Attributes[c2$15187102] = {Temporary}
 
c2$15187102 = {{rp$15187223[t1$15187223[#1]], t1$15187223[#1]} & , 
     {rm$15187223[t2$15187223[#1]], t2$15187223[#1]} & }
 
Attributes[rp$15187223] = {Temporary}
 
rp$15187223[t$_] := \[Rho] /. s$15187223[[2]] /. \[Tau] -> t$
 
Attributes[s$15187223] = {Temporary}
 
s$15187223 = {{\[Rho] -> 0.5*(4.*Cos[0.6666666666666666*(0. + \[Tau])] - 
         1.*Sqrt[-12. + 16.*Cos[0.6666666666666666*(0. + \[Tau])]^2])}, 
     {\[Rho] -> 0.5*(4.*Cos[0.6666666666666666*(0. + \[Tau])] + 
         Sqrt[-12. + 16.*Cos[0.6666666666666666*(0. + \[Tau])]^2])}}
 
Attributes[t1$15187223] = {Temporary}
 
t1$15187223[t$_] := tr$15187223 + (tl$15187223 - tr$15187223)*t$
 
Attributes[tr$15187223] = {Temporary}
 
tr$15187223 = -0.7853981633974483
 
Attributes[tl$15187223] = {Temporary}
 
tl$15187223 = 0.7853981633974483
 
Attributes[rm$15187223] = {Temporary}
 
rm$15187223[t$_] := \[Rho] /. s$15187223[[1]] /. \[Tau] -> t$
 
Attributes[t2$15187223] = {Temporary}
 
t2$15187223[t$_] := tl$15187223 + (tr$15187223 - tl$15187223)*(t$ - 1)
 
Attributes[b11$15187102] = {Temporary}
 
b11$15187102 = {t, 1/400000000, 399999999/400000000}
 
Attributes[b21$15187102] = {Temporary}
 
b21$15187102 = {u, 1/400000000, 399999999/400000000}
 
Attributes[acc$15187102] = {Temporary}
 
acc$15187102 = 8
 
Attributes[j22$15187102] = {Temporary}
 
j22$15187102 = Sqrt[0.27415567780803773*
       (4.*Cos[0.6666666666666666*(0.7853981633974483 - 1.5707963267948966*
              (-1 + u))] - 1.*Sqrt[-12. + 16.*Cos[0.6666666666666666*
                (0.7853981633974483 - 1.5707963267948966*(-1 + u))]^2])^2 + 
      0.25*(4.1887902047863905*Sin[0.6666666666666666*(0.7853981633974483 - 
             1.5707963267948966*(-1 + u))] - (16.755160819145562*
           Cos[0.6666666666666666*(0.7853981633974483 - 1.5707963267948966*(
                -1 + u))]*Sin[0.6666666666666666*(0.7853981633974483 - 
              1.5707963267948966*(-1 + u))])/
          Sqrt[-12. + 16.*Cos[0.6666666666666666*(0.7853981633974483 - 
                 1.5707963267948966*(-1 + u))]^2])^2]
 
Attributes[b22$15187102] = {Temporary}
 
b22$15187102 = {u, 400000001/400000000, 799999999/400000000}

